Two-Stage Random Alternation Framework for One-Shot Pansharpening

Deep learning has substantially advanced pansharpening, achieving impressive fusion quality. However, a prevalent limitation is that conventional deep learning models, which typically rely on training datasets, often exhibit suboptimal generalization to unseen real-world image pairs. This restricts their practical utility when faced with real-world scenarios not included in the training datasets. To overcome this, we introduce a two-stage random alternating framework (TRA-PAN) that performs instance-specific optimization for any given Multispectral(MS)/Panchromatic(PAN) pair, ensuring robust and high-quality fusion. TRA-PAN effectively integrates strong supervision constraints from reduced-resolution images with the physical characteristics of the full-resolution images. The first stage introduces a pre-training procedure, which includes Degradation-Aware Modeling (DAM) to capture spectral degradation mappings, alongside a warm-up procedure designed to reduce training time and mitigate the adverse effects of reduced-resolution data. The second stage employs Random Alternation Optimization (RAO), randomly alternating between reduced- and full-resolution images to refine the fusion model progressively. This adaptive, per-instance optimization strategy, operating in a one-shot manner for each MS/PAN pair, yields superior high-resolution multispectral images. Experimental results demonstrate that TRA-PAN outperforms state-of-the-art (SOTA) methods in quantitative metrics and visual quality in real-world scenarios, underscoring its enhanced practical applicability and robustness.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

$pdflatex = 'pdflatex %O %S; ps2pdf14 -dPDFSETTINGS=/prepress %B.pdf %B-embed.pdf; mv %B-embed.pdf %B.pdf';

==> tables/exp_SOTA_compar_Reduce.tex <==
\begin{table*}[h]
\centering
\caption{Comparisons on WV3, QB, and GF2 reduced-resolution datasets, each with 20 samples. Best:\textbf{bold} , and second-best: \underline{underline}.}
\vspace{-0.1cm}
\begin{tabular}{cc@{\hskip 3pt}c@{\hskip 0.005in}c@{\hskip 0.005in}cc@{\hskip 3pt}c@{\hskip 0.005in}c@{\hskip 0.005in}cc@{\hskip 3pt}c@{\hskip 0.005in}c@{\hskip 0.005in}c}
\hline
\vspace{-3pt}
\multirow{2}{*}{\textbf{Methods}} & \multicolumn{4}{c}{\textbf{ WV3 }} & \multicolumn{4}{c}{\textbf{QB}} & \multicolumn{4}{c}{\textbf{GF2}}\\ 
\cmidrule(lr){2-5}  \cmidrule(lr){6-9}  \cmidrule(lr){10-13}  
 & \textbf{PSNR$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} & \textbf{Q8$\uparrow$}& \textbf{PSNR$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} & \textbf{Q4$\uparrow$} & \textbf{PSNR$\uparrow$} & \textbf{SAM$\downarrow$} & \textbf{ERGAS$\downarrow$} &\textbf{Q4$\uparrow$} 
\\ \hline
MTF-GLP-FS~\cite{MTF-GLP-FS} &32.963 & 5.316 & 4.700 & 0.833  & 32.709 & 7.792 & 7.373 &0.835 & 35.540 & 1.655 & 1.589 & 0.897
\\  
BDSD-PC~\cite{BDSD-PC} &32.970 & 5.428 & 4.697 & 0.829 & 32.550 & 8.085 & 7.513 &0.831 & 35.180 & 1.681 & 1.667 & 0.892 
\\ 
TV~\cite{TV} & 32.381 & 5.692 & 4.855 & 0.795& 32.136 & 7.510 & 7.690 &0.821 & 35.237 & 1.911 & 1.737 & 0.907 
\\ \hline

PNN~\cite{PNN} & 37.313 & 3.677 & 2.681 & 0.893  & 36.942 & 5.181 & 4.468 &0.918 & 39.071 & 1.048 & 1.057 & 0.960 
\\ 
PanNet~\cite{Yang2017PanNet} &37.346 & 3.613 & 2.664 & 0.891  & 34.678 & 5.767 & 5.859 &0.885& 40.243 & 0.997 & 0.919 & 0.967
\\ 
DiCNN~\cite{hePansharpeningDetailInjection2019} & 37.390 & 3.592 & 2.672 & 0.900 & 35.781 & 5.367 & 5.133 & 0.904 & 38.906 & 1.053 & 1.081 & 0.959 \\ 
FusionNet~\cite{FusionNet} & 38.047 & 3.324 & 2.465 & 0.904 & 37.540 & 4.904 & 4.156 &0.925 & 39.639 & 0.974 & 0.988 & 0.964 
\\ 
LAGNet~\cite{LAGConv}& 38.592& 3.103& 2.291& 0.910& 38.209& 4.534& 3.812&\underline{0.934}& 42.735& 0.786& 0.687& 0.980
\\ 
LGPNet~\cite{zhao2023lgpconv}& 38.147& 3.270& 2.422& 0.902& 36.443& 4.954& 4.777& 0.915& 41.843& 0.845& 0.765&  0.976
\\ 
PanMamba~\cite{He2024PanMambaEP} & \underline{39.012}& \textbf{2.913}& \underline{2.184}& \underline{0.920} & 37.356 & 4.625 & 4.277 &0.929 & 42.907 & 0.743& 0.684 & 0.982
\\ 
% HMPNet&0& 38.765& 3.063& 2.230& 0.916& \textbf{39.227}& 4.617& \textbf{3.404}& 0.936& \textbf{45.926}& 0.782& \textbf{0.537}& \underline{0.985}\\
%  ZS-Pan~\cite{caoif2024} & 39.001       & 2.938& 2.192& 0.918
%  &\underline{38.211}& \underline{4.512}&  \underline{3.807}&0.930& 
%  \underline{43.286}& \underline{0.715}& \underline{0.634}&\underline{0.983}
% \\ 
 
 \textbf{Proposed} & \textbf{39.170}& \textbf{2.913}& \textbf{2.145}& \textbf{0.921}& \textbf{38.466}& \textbf{4.450}& \textbf{3.705}&\textbf{0.937}& \textbf{43.884}& \textbf{0.672}& \textbf{0.597}& \textbf{0.985} \\ \hline
\end{tabular}
%\caption{Comparisons on WV3, QB, and GF2 reduced-resolution datasets, each with 20 samples, respectively. Best: bold, and second-best: underline.}
\label{tab:all_reduce}
\vspace{-0.4cm}
\end{table*}


==> tables/netchange.tex <==
\begin{table}[t]
\centering
\caption{Experiment of different backbones in WV3 dataset.}
\setlength{\tabcolsep}{4pt} % 默认值为6pt，调整为4pt以缩短列间距
\centering
\begin{tabular}{cccc}
\hline
\multirow{2}{*}{\textbf{Backbone}} & \multicolumn{3}{c}{\textbf{WV3}} \\
\cmidrule(lr){2-4}
& \textbf{D$_\lambda \downarrow$} & \textbf{D$s$$\downarrow$} & \textbf{HQNR$\uparrow$} \\
\hline
TRA-PAN  & 0.0193  & 0.0154 & 0.9657 \\
LAG  & 0.0939  &  0.1065 &  0.8103  \\
LGP & 0.0710 & 0.1408  & 0.7988  \\
\hline
\end{tabular}
\label{table:Backbone}
\end{table}

==> tables/suppl_method.tex <==
\begin{table*}[t]
\centering
\vspace{-0.3cm}
\caption{Introduction for pansharpening methods involved in the benchmark.}
\label{tab:methods}
\vspace{-0.1cm}
\begin{tabular}{@{\hskip 3pt}l@{\hskip 3pt}c@{\hskip 3pt}c@{\hskip 3pt}l@{\hskip 3pt}}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Category}} & \multirow{2}{*}{\textbf{Year}} & \multirow{2}{*}{\textbf{Introduction}} \\
\hline
EXP~\cite{EXP} & & 2002 & Simply upsamples the MS image. \\
MTF-GLP-FS~\cite{vivoneFullScaleRegressionBased2018} & MRA & 2018 & Estimates the injection coefficients at full resolution rather than reduced resolution. \\
TV~\cite{palssonNewPansharpeningAlgorithm2014} & VO & 2013 & Employs total variation as a regularization technique for addressing an ill-posed problem defined by a commonly utilized explicit model for image formation. \\
BDSD-PC~\cite{vivoneRobustBandDependentSpatialDetail2019} & CS & 2018 & Addresses the limitations of the band-dependent spatial-detail (BDSD) method in images with more than four spectral bands. \\
CVPR2019~\cite{fuVariationalPanSharpeningLocal2019} & VO & 2019 & Integrates a more precise spatial preservation strategy by considering local gradient constraints within distinct local patches and bands. \\
LRTCFPan~\cite{LRTCFPan} & VO & 2023 & Utilizes low-rank tensor completion (LRTC) as the foundation and incorporating various regularizers for enhanced performance. \\
PNN~\cite{masiPansharpeningConvolutionalNeural2016a} & ML & 2016 & The first convolutional neural network (CNN) for pansharpening with three convolutional layers. \\
PanNet~\cite{yangPanNetDeepNetwork2017} & ML & 2017 & Deeper CNN for pansharpening. \\
DiCNN~\cite{hePansharpeningDetailInjection2019} & ML & 2019 & Introduces the detail injection procedure into pansharpening CNNs. \\
FusionNet~\cite{dengDetailInjectionBasedDeep2021} & ML & 2021 & Combines ML techniques with traditional fusion schemes like CS and MRA. \\
DCFNet~\cite{wuDynamicCrossFeature2021} & ML & 2021 & Considers the connections of information between high-level semantics and low-level features through the incorporation of multiple parallel branches. \\
MMNet~\cite{mmnet} & ML & 2022 & A model-driven deep unfolding network with memory-augmentation. \\
LAGConv~\cite{jinLAGConvLocalContextAdaptive2022} & ML & 2022 & Adaptive convolution with enhanced ability to leverage local information and preserve global harmony. \\
HMPNet~\cite{hmpnet} & ML & 2023 & An interpretable model-driven deep network tailored for the fusion of hyperspectral (HS), multispectral (MS), and panchromatic (PAN) images. \\
\hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}


==> tables/timetable.tex <==


\begin{table*}[t]
\centering
\caption{Running Time (seconds) comparison on the WV3 dataset (20 samples), split into two rows.}
\begin{tabular}{lccccc} % Adjust the number of 'c' columns based on the larger group (here 5)
\toprule
\textbf{Metric} & \textbf{MTF-GLP-FS} & \textbf{BDSD-PC} & \textbf{TV} & \textbf{FusionNet} & \textbf{LAGNet} \\
\cmidrule(lr){2-6} % Rule for the first group of methods
Time (s) on WV3 & tbd & tbd & tbd & tbd & tbd \\
\midrule % Separator between the two rows of methods
% Added the metric description in the first column of the second row as requested
\textbf{Metric} & \textbf{LGPNet} & \textbf{CANNet} & \textbf{ZS-Pan} & \textbf{PanMamba} & \textbf{Proposed} \\
\cmidrule(lr){2-6} % Rule for the second group of methods
Time (s) on WV3 & tbd & tbd & tbd & tbd & \textbf{tbd} \\ % Note: Proposed value also marked tbd
\bottomrule
\end{tabular}
\label{tab:RunningTimeWV3_double_row_filled} % Updated label
\end{table*}


